On the explainable properties of 1-Lipschitz Neural Networks: An Optimal Transport Perspective

Input gradients have a pivotal role in a variety of applications, including adversarial attack algorithms for evaluating model robustness, explainable AI techniques for generating Saliency Maps, and counterfactual explanations.However, Saliency Maps generated by traditional neural networks are often noisy and provide limited insights. In this paper, we demonstrate that, on the contrary, the Saliency Maps of 1-Lipschitz neural networks, learned with the dual loss of an optimal transportation problem, exhibit desirable XAI properties:They are highly concentrated on the essential parts of the image with low noise, significantly outperforming state-of-the-art explanation approaches across various models and metrics. We also prove that these maps align unprecedentedly well with human explanations on ImageNet.To explain the particularly beneficial properties of the Saliency Map for such models, we prove this gradient encodes both the direction of the transportation plan and the direction towards the nearest adversarial attack. Following the gradient down to the decision boundary is no longer considered an adversarial attack, but rather a counterfactual explanation that explicitly transports the input from one class to another. Thus, Learning with such a loss jointly optimizes the classification objective and the alignment of the gradient, i.e. the Saliency Map, to the transportation plan direction.These networks were previously known to be certifiably robust by design, and we demonstrate that they scale well for large problems and models, and are tailored for explainability using a fast and straightforward method.

==> partsv2/conclusion_otml.tex <==
In this paper, we study the explainability properties of OTNN~(Optimal Transport Neural Networks) 
that are 1-Lipschitz~constrained neural networks trained with an optimal transport dual loss. 
We establish that the gradient of the optimal solution aligns with the transportation plan direction,
and the closest decision boundary point (adversarial example) also lies in this gradient direction at a distance of the absolute value of the network output.  
Relying on a formal definition of Optimal Transport counterfactuals, we build a link between the OTNN gradients and counterfactual explanations
%, justifying that 
. We thus show that
OTNNs loss jointly targets the classification task and induces a gradient alignment to the transportation plan. 
%building a counterfactual explanation. 
%%%%%%These beneficial properties of the gradient substantially enhance the Saliency Map XAI method for \otnn~s.
The experiments show that the simple Saliency Map has top-rank scores on state-of-the-art XAI metrics, and largely outperforms any method applied to unconstrained networks. 
%This is illustrated in the experiments which shows that the simple Saliency Map for OTTNs has top-rank scores on state-of-the-art XAI metrics, and largely outperforms any method applied to unconstrained networks. 
%Besides, as far as we know, our models are the first large provable 1-Lipschitz neural models that match state-of-the-art results on large problems.
%To the best of our knowledge, our models are also the first large, provable 1-Lipschitz neural models that achieve results on-par with state-of-the-art on large problems. 
And even if counterfactual explanations are less compelling for Imagenet, probably due to the complexity of transport for 
large number of classes,
%multiclass
 we prove that \otnn s Saliency Maps are impressively aligned to human explanations. 

This paper demonstrates how leveraging an Optimal Transport (OT) objective for classification tasks provides additional interesting properties for critical problems. 
%1-Lipschitz Neural Networks are known for their certifiable robustness; But, Optimal Transport Neural Networks (OTNNs) offer inherent explainability by design through the utilization of the simple Saliency Map method.
Besides the well known certifiable robustness of 1-Lipschitz Neural Networks, Optimal Transport Neural Networks (OTNNs) offer inherent explainability by design through the utilization of the simple Saliency Map method.
%—and is notably aligned with human rationales. 
Furthermore, our study reveals that OTNNs can achieve accuracy comparable to those of unconstrained networks.
While the training duration for OTNNs is three to six times longer than that for unconstrained networks, they share comparable computational costs for inference. We hope that this contribution will further add to the growing interest in the application of Optimal Transport for Neural Networks.


%We first provide  enhancements of the \losshkr, proposed in\cite{serrurier2021achieving}, reducing the number of hyperparameters and the improving the performances at convergence. 
%Experiments provide quantitative and qualitative evaluations showing that Saliency Maps for OTNNs have better score than for unconstrained networks, and comparable scores to other XAI methods.To end with we show that Saliency Maps for OTNNs have an unprecedented alignment to human explanations.   
%OTNNs, because of their connection with optimal transport, structurally produce counterfactual explanations. Indeed, we prove that the gradient of an OTNN at a point represents the direction of the adversarial attack but also of its image in the optimal transport plan, transforming the adversary attacks into an understandable counterfactual explanation.  
%This is illustrated in the experiment which shows that the simple Saliency Map for OTTNs has top-rank scores on state-of-the-art XAI metrics, and largely outperforms any method applied to unconstrained networks.\commentgreen{Last but not least, we prove that \otnn s Saliency Maps are impressively aligned to human explanations.} 

%\commentgreen{peut etre renommer pour ne pas trop faire post neurips, et developper les points negatifs de notre methode -voir reponse au reviewer-}

==> partsv2/experiment_otml.tex <==
We conduct experiments with networks learnt on FashionMNIST~\cite{Xiao2017FashionMNIST}, and 22 binary labels of CelebA~\cite{liu2015faceattributes} datasets, Cat vs Dog (binary classification, 224x224x3 uncentered images),  and Imagenet~\cite{imagenet}. Note that labels in CelebA are very unbalanced (see~Table~2 in Appendix~A.2, with for instance less than $5\%$ samples for \textit{Mustache} or \textit{Wearing\_Hat}).% or \textit{Wearing\_Hat}). 
Architectures used for \otnn s~and unconstrained networks are similar (same number of layers and neurons, a VGG for FashionMNIST and CelebA, a ResNet50 for Cat vs Dog and Imagenet). We also train an alternative of ResNet50 OTNN with twice the number of parameters (50 M).  Unconstrained networks use batchnorm and ReLU layers for activation, whereas \otnn s~only use GroupSort2~\cite{pmlr-v97-anil19a,serrurier2021achieving} activation. \otnn s~are built using the \Deellip library.  
%*Loss
The loss functions are cross-entropy for unconstrained networks (categorical for multiclass, and sigmoid for multilabel settings), and hKR \losshkr~(and the multiclass variants see appendix A.2.3) for \otnn s. We train all networks with Adam optimizer~\cite{Diederik14Adam}. Details on architectures and parameters are given in Appendix~A.2.


\textbf{Classification performance:} \otnn~models achieve comparable results to  unconstrained ones, confirming claims of~\cite{bethunelip}: they reach 88.5\%
%\commentgreen{@Mathieu merci de remplir}
average accuracy on FashionMNIST
(Table~6), and 81\% (resp. 82\%) average Sensitivity (resp. Specificity) over labels on CelebA (Table~6 in Appendix~A.3). We use  Sensitivity and Specificity for CelebA to take into consideration the unbalanced labels. \otnn s~achieve 96\%  accuracy (98\% for the unconstrained version) on Cat vs Dog and 67\% (75\% for the unconstrained version) on Imagenet. The ResNet50 OTNN with 50M parameters achieves 70\% accuracy on Imagenet. 

%\subsection{Quantitative evaluation of explanations metrics}
\input{partsv2/megatab_otml}
\input{partsv2/explanations_otml}
%Reseau normal: Grad => metriques nulles; comparer avec autre methode d'explication
%Reseau hKR: Grad => metriques++; eventuellement comparer autres explications 
%Metriques: robustnes-Sr; stability; .... (voir avec thomas les autres potentiellement deja dans xplique qu'on pourrait tester )
%\subsection{adult} explaination show unfairness

\textbf{Qualitative results: }
\input{partsv2/qualitative_results_otml}

==> partsv2/experiments.tex <==
e conduct experiments networks learnt on FashionMNIST~\cite{Xiao2017FashionMNIST}, and 22 binary labels of CelebA~\cite{liu2015faceattributes} datasets\commentgreen{, and Imagenet~\cite{imagenet}}. Note that labels in CelebA are very unbalanced (see~Table~\ref{tab:celebA_stats} in Appendix~\ref{ann:complementary_results}, with for instance less than $5\%$ samples for \textit{Mustache} or \textit{Wearing\_Hat}).% or \textit{Wearing\_Hat}). 

\sout{A VGG-like architecture~\cite{Parkhi15VGG} is used, with equivalent linear layer sizes for \otnn s~and unconstrained networks (same number of layers and neurons).}\commentgreen{Architectures used for \otnn s~and unconstrained networks are similar (same number of layers and neurons).} Unconstrained networks use batchnorm and ReLU layers for activation, whereas \otnn s~only use GroupSort2~\cite{pmlr-v97-anil19a,serrurier2021achieving} activation. \otnn s~are built using the \Deellip library.
%*Loss
The loss functions are cross-entropy for unconstrained networks (categorical for multiclass, and sigmoid for multilabel settings), and hKR \losshkr~(and the proposed variants) for \otnn s. We train all networks with ADAM optimizer~\cite{Diederik14Adam}. Details on architectures and parameters are given in Appendix~\ref{ann:parameters}.


\textbf{Classification performance:} \otnn~models achieve comparable results to  unconstrained ones, confirming claims of~\cite{bethunelip}: they reach 88.5\%
%\commentgreen{@Mathieu merci de remplir}
average accuracy on FashionMNIST
(Table~\ref{tab:fashion_results}), and 81\% (resp. 82\%) average Sensitivity (resp. Specificity) over labels on CelebA (Table~\ref{tab:celebA_results} in Appendix~\ref{ann:complementary_results}). We use  Sensitivity and Specificity for CelebA to take into consideration the unbalanced labels. \commentgreen{Concerning Imagenet, \otnn~performances ......}






\subsection{Quantitative evaluation of explanations metrics}
\input{parts/explanations_metrics}
%Reseau normal: Grad => metriques nulles; comparer avec autre methode d'explication
%Reseau hKR: Grad => metriques++; eventuellement comparer autres explications 
%Metriques: robustnes-Sr; stability; .... (voir avec thomas les autres potentiellement deja dans xplique qu'on pourrait tester )
%\subsection{adult} explaination show unfairness

\subsection{Qualitative results}
\input{parts/qualitative_results}

==> partsv2/explanations_otml.tex <==
We present the results of quantitative evaluations of XAI metrics to compare the Saliency Map method with other explanation methods on \otnn, and more generally compare XAI explanations methods on these networks and their unconstrained counterparts. On CelebA, we only present  the results for the label \textit{Mustache}, but results for the other labels are similar. Parameters for explanation methods and metrics are given in Appendix~A.4. We have chosen to present in Table \ref{table:xaimetric}  two SoTA XAI metrics that enable comparison between \otnn s~and unconstrained networks.  \textbf{$\mu\text{Fidelity}$ metric}~\cite{Bhatt20muFidelity} is a well-known method that measures the correlation between important variables defined by the explanation method and the model score decreases when these variables are reset to a baseline state (or replaced by uniform noise). Another important property for explanations is their stability for nearby samples. In~\cite{Yeh19InfidelityExplain}, the authors proposed Stability metrics based on the $L_2$ distance. To better evaluate this stability and make it comparable for different models, we replace the $L_2$ distance by $1-\rho$, $\rho$ being the Spearman rank correlation. Other model-dependent metrics are described in the Appendix. Results from the 50M parameter ResNet \otnn~are included in the human alignment study (Fig~\ref{fig:human_alignement}) to illustrate that enhancing the model's complexity can bolster both the accuracy and alignment. The following observations can be drawn from Table \ref{table:xaimetric}:
\iffalse
\subsubsection{Saliency Maps on \otnn~become reliable explanations}
\commentgreen{on s'etait fait critiqué sur des termes comme trusworrthy et reliable je pense qu'il faudrait changer ce titre de section: tentatives: \\
Enhanced scores for OTNNs Saliency Maps\\
%Good properties of OTNNs saleicy maps
\\
....
Ok vu tu supprime tout ca vu qu'il n'y a plus la tablleau
}
\fi

%\textbf{Insertion and Deletion metrics:} We first assess the quality of  Saliency Map explanations for the proposed network using Insertion and Deletion metrics~\cite{petsiuk18Rise}. Classical explanation methods, including the Saliency Map, are evaluated on CelebA and FashionMNIST datasets for both types of networks. Even if the score values cannot be compared between different networks, Table~\ref{tab:ins_del_metric} shows the Saliency Map method becomes competitive on these metrics and matches the top-ranking methods, whereas it is not the case for unconstrained networks. In Annex~\ref{ann:explanation_metrics}, we show that it is also the case for other metrics such as Robustness-SR~\cite{HsiehYLRKKH21}.

%\commentgreen{la parie deletion-insertion 0 c'est vraiment pas clair je pense qu'il faut l'enlever. On peut remplacer par robustnessSR si on arrive a faire FashionMNIST}.

% \iffalse
% \fel{Proposition: j'ai corrigé quelques typos dans la table et essayé de séparer des parties. Je ne suis pas sur que ce soit mieux, je laisse les deux et vous choisirez ;)}
% \begin{table}
%   \caption{Insertion and Deletion metrics evaluation; GC: GradCam, GI: Gradient.Input, IG: Integrated Gradient, Saliency Rk : Rank}
%   \label{tab:ins_del_metric_2}
%   \centering
%   \begin{tabular}{lc|cccccc}
%     \toprule
% Dataset& Network&  \multicolumn{6}{c}{Deletion-Uniform (lower is better)}  \\
% & & GC & GI & IG & Rise& Saliency& SmoothGrad\\
%  \midrule
% CelebA& \otnn & 9.41& 9.38& 9.36& 8.89& 8.32 (Rk2) & \textbf{8.28}\\
% & Unconstrained& 5.13& 3.33& \textbf{3.18}& 3.61& 3.50 (Rk4) & 3.41\\
% Fashion-& \otnn& 0.23& 0.28& 0.28& 0.24& 0.22 (Rk2) & \textbf{0.21}\\
% MNIST & Unconstrained& 0.32& 0.35& 0.39& 0.32& 0.26 (Rk2) & \textbf{0.24}\\
%  \midrule
% & &  \multicolumn{6}{c}{Insertion Uniform (higher is better)} \\
% CelebA& \otnn& 10.25& 10.44& 10.50& 10.46& \textbf{11.29} (Rk1) & 11.28\\
% & Unconstrained& 9.43& 8.45& 9.24& \textbf{12.20} & 6.71 (Rk6) & 6.72\\
% Fashion-& \otnn& \textbf{0.28}& 0.20& 0.20& 0.26& 0.25 (Rk4) & 0.26\\
% MNIST & Unconstrained& \textbf{0.44} & 0.32& 0.26& 0.40& 0.30 (Rk4)& 0.24\\
%     \bottomrule
%     \end{tabular}
% \end{table}
% \fi 



%whatever the explanation method, the $\mu\text{Fidelity}$, with zero or uniform score modification, is significantly higher when it is applied on \otnn. There are instances where this is not the case for the ResNet architecture; however, in such cases, the Saliency Map of OTNN significantly outperforms any attribution metrics for unconstrained models. 
%This confirms and amplify the result ~\cite{felHowGood22}, which shows that \onlyonelip~ neural networks, for the two proposed metrics, produce explanations with higher scores than common neural networks (\mathieu{A améliorer}). 
A similar observation 
holds for 
%applies to 
the Stability Spearman rank
: \otnn~scores are better whatever the attribution method.
%, where the score is substantially better for \otnn, regardless the attribution considered.

\iffalse
\begin{figure*}
\begin{tabular}{@{}c@{}cc@{}}
\centering
    \begin{tabular}{c}
  \rowcolor{white}  \rotatebox{90}{\textbf{Saliency}}
  \end{tabular} & 
  \begin{tabular}{@{}l@{}l@{}l@{}}
    \includegraphics[width=.15\linewidth]{img/saliency_smoothgrad/saliency_1Lip_3_crop.png} &
  \includegraphics[width=.15\linewidth]{img/catvsdog/OTNN_saliency_1.jpg} & 
  \includegraphics[width=.15\linewidth]{img/imagenet/OTNN_saliency_2.jpg}
  \end{tabular} & 
  \begin{tabular}{@{}l@{}l@{}l@{}}
  \includegraphics[width=.15\linewidth]{img/saliency_smoothgrad/saliency_Unconst_3_crop.png} &
  \includegraphics[width=.15\linewidth]{img/catvsdog/resnet50_saliency_1.jpg} & 
  \includegraphics[width=.15\linewidth]{img/imagenet/resnet50_saliency_2.jpg}
  \end{tabular}\\

  \begin{tabular}{l}
   \rotatebox{90}{\textbf{SmoothGrad}} 
  \end{tabular} &
  \begin{tabular}{@{}l@{}l@{}l@{}} \includegraphics[width=.15\linewidth]{img/saliency_smoothgrad/smoothgrad_1Lip_3_crop.png} &\includegraphics[width=.15\linewidth]{img/catvsdog/OTNN_smooth_1.jpg} & \includegraphics[width=.15\linewidth]{img/imagenet/OTNN_smooth_2.jpg}
  \end{tabular} & 
  \begin{tabular}{@{}l@{}l@{}l@{}}
  \includegraphics[width=.15\linewidth]{img/saliency_smoothgrad/smoothgrad_Unconst_3_crop.png} & \includegraphics[width=.15\linewidth]{img/catvsdog/resnet50_smooth_1.jpg} & \includegraphics[width=.15\linewidth]{img/imagenet/resnet50_smooth_2.jpg}
  \end{tabular}\\
& (a)~\otnn
  &  (b) Unconstrained
\end{tabular}
\caption{Comparison of Saliency Map and SmoothGrad  explanations for (a) \otnn~ and (b) unconstrained network for, from left to right, CelebA, Cat vs Dog and Imagenet datasets.} %\commentgreen{Thomas a donné des nouvelles images elles sont dans saliency_smoothgrad/robust... a mettre en annexe ou ici }}
\label{fig:saliency_smoothgrad}
\end{figure*}
\fi

\iffalse
\begin{figure*}
\begin{tabular}{@{}c@{}c@{}c}
\centering
  \begin{tabular}{l}
    \rotatebox{90}{\textbf{Saliency}}
  \end{tabular}
 & 
  \begin{tabular}{@{}l@{}l@{}l}
    \includegraphics[width=.14\linewidth]{img/saliency_smoothgrad/saliency_1Lip_3_crop.png} &
  \includegraphics[width=.15\linewidth]{img/catvsdog/OTNN_saliency_1.jpg} %& 
%  \includegraphics[width=.15\linewidth]{img/imagenet/OTNN_saliency_2.jpg}
  \end{tabular} &
  \multirow{6}{c}{\includegraphics[width=.35\textwidth]{img/human_alignment.jpg}}
  \\

  \begin{tabular}{l}
   \rotatebox{90}{\textbf{SmoothGrad}} 
  \end{tabular} &
  \begin{tabular}{@{}l@{}l@{}l} \includegraphics[width=.14\linewidth]{img/saliency_smoothgrad/smoothgrad_1Lip_3_crop.png} &\includegraphics[width=.15\linewidth]{img/catvsdog/OTNN_smooth_1.jpg} %& \includegraphics[width=.15\linewidth]{img/imagenet/OTNN_smooth_2.jpg}
  \end{tabular} &  \\
& (a)~\otnn  & \\
  \begin{tabular}{l}
    \rotatebox{90}{\textbf{Saliency}}
  \end{tabular}
 & 
  \begin{tabular}{@{}l@{}l@{}l}
  \includegraphics[width=.15\linewidth]{img/saliency_smoothgrad/saliency_Unconst_3_crop.png} &
  \includegraphics[width=.16\linewidth]{img/catvsdog/resnet50_saliency_1.jpg} %& 
%  \includegraphics[width=.15\linewidth]{img/imagenet/resnet50_saliency_2.jpg}
  \end{tabular}  & \\
  \begin{tabular}{l}
   \rotatebox{90}{\textbf{SmoothGrad}} 
  \end{tabular} &
  \begin{tabular}{@{}l@{}l@{}l}
  \includegraphics[width=.15\linewidth]{img/saliency_smoothgrad/smoothgrad_Unconst_3_crop.png} & \includegraphics[width=.16\linewidth]{img/catvsdog/resnet50_smooth_1.jpg} %& \includegraphics[width=.15\linewidth]{img/imagenet/resnet50_smooth_2.jpg}
  \end{tabular} & \\
&   (b) Unconstrained& 
\end{tabular}
\caption{Comparison of Saliency Map and SmoothGrad  explanations for (a) \otnn~ and (b) unconstrained network for the respectively CelebA, cat vs dog and imagenet.} %\commentgreen{Thomas a donné des nouvelles images elles sont dans saliency_smoothgrad/robust... a mettre en annexe ou ici }}
\label{fig:saliency_smoothgrad}
\end{figure*}
\fi
%\textbf{Saliency Map on \otnn~are less complex:} 
%Complexity of a given explanation is linked to the understandability by a human. \commentgreen{Thomas si tu as des references ? TBC should be kolmogorov but JPEG is a good surrogate}
%Inspired by previous works~\cite{da2011image} highlighting a strong correlation between Kolmogorov complexity and human evaluation of complexity~\cite{forsythe2008confounds,forsythe2009visual}. We used a JPEG based compressor~\cite{vereshchagin2005lossy} as a simple approximation of  visual explanation complexity~\cite{li2004similarity}: \otnn s~yield simpler explanations than unconstrained networks in all case. %($16.8kB$) -see Figure~\ref{fig:saliency_smoothgrad} for a qualitative comparison-.
%. \commentgreen{il manque les resultats (a faire Franck)}



%\subsubsection{\otnn s~ provide better explanations}
%\commentgreen{idem better ca veut pas dire grand chose\\
%\otnn s~ explanations exhibit more fidelity and stability\\
%...\\
%d'autres propositions?}





\textbf{\otnn s~ explanations are aligned with human ones : }
Adopting the method presented in~\cite{linsley2017visual}, using the ClickMe dataset, we compute the human feature alignment of OTNN Saliency Maps and compare with the others models tested in ~\cite{ fel2022aligning}-- more than 100 recent deep neural networks. In Figure ~\ref{fig:human_alignement}, we demonstrate that 
OTNN models Saliency Maps, %the Saliency Map of  the OTNN model,
which also carries a theoretical interpretation as the direction of the transport plan,  is more aligned with human attention than any other tested models and significantly surpasses the Pareto front discovered by~\cite{fel2022aligning}. The OTNN model is even more aligned than a ResNet50 model trained with a specific alignment objective, proposed by~\cite{fel2022aligning}, and called \textit{Harmonized ResNet50}. 
This finding is interesting as it indicates \otnn s are less prone to relying on spurious correlations~\cite{geirhos2020shortcut} and 
%is more adept at capturing 
better capture
human visual strategies for object recognition.
%The implications of these findings are crucial first for cognitive science: A model with closer alignment with human attention and visual strategies can provide a more comprehensive understanding of how vision operates for humans. Besides, it enhances the predictability, interpretability, and performance of object recognition models which as positive consequences in industry settings.
The implications of these results are crucial for both cognitive science and industrial applications. A model that more closely aligns with human attention and visual strategies can provide a more comprehensive understanding of how vision operates for humans, and also enhance the predictability, interpretability, and performance of object recognition models in industry settings. 
Furthermore, the drop in alignment observed in recent models highlights the necessity of considering the alignment of model visual strategies with human attention while developing object recognition models to reduce the reliance on spurious correlations and ensure that our models get things right for the right reasons.

\iftrue
\begin{figure*}
\centering
\includegraphics[width=.99\textwidth]{img/human_alignment_flat_2.pdf}
\caption{\textbf{\otnn~are aligned with Human attention.} Our study shows that the Saliency Map of OTNN model is highly aligned with human attention.% This finding is supported by the work of~\cite{fel2022aligning}, which demonstrates the trade-off between deep neural network (DNN) performance and alignment with human feature importance from the ClickMe~\cite{linsley2017visual} dataset. The degree of alignment between human and DNN saliency is measured using the mean Spearman correlation, normalized by the average inter-rater alignment of humans. 
%Among the hundreds of model tests performed in the original study, our model is the only one that breaks the Pareto front, suggesting a superior trade-off between DNN performance and alignment with human attention. Even an Harmonized model from~\cite{fel2022aligning} study, which was specifically designed to predict human attention, achieves a lower alignment than our model. \fel{on peut remove ca si vous voulez:} Overall, our results highlight the potential of the OTNN model to capture the visual strategies used by humans for object recognition, and may lead to improved performance and interpretability of object recognition models in both cognitive science and industry applications.
}
\label{fig:human_alignement}
\end{figure*}
\fi



\iffalse
\begin{figure*}
\centering
\includegraphics[width=.5\textwidth]{img/human_alignment.jpg}
\caption{\textbf{\otnn~are aligned with Human attention.} Our study shows that the Saliency Map of \otnn~model is highly aligned with human attention.% This finding is supported by the work of~\cite{fel2022aligning}, which demonstrates the trade-off between deep neural network (DNN) performance and alignment with human feature importance from the ClickMe~\cite{linsley2017visual} dataset. The degree of alignment between human and DNN saliency is measured using the mean Spearman correlation, normalized by the average inter-rater alignment of humans. 
%Among the hundreds of model tests performed in the original study, our model is the only one that breaks the Pareto front, suggesting a superior trade-off between DNN performance and alignment with human attention. Even an Harmonized model from~\cite{fel2022aligning} study, which was specifically designed to predict human attention, achieves a lower alignment than our model. \fel{on peut remove ca si vous voulez:} Overall, our results highlight the potential of the OTNN model to capture the visual strategies used by humans for object recognition, and may lead to improved performance and interpretability of object recognition models in both cognitive science and industry applications.
}
\label{fig:human_alignement}
\end{figure*}
\fi

==> partsv2/megatab_otml.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{lllllllll}
\cline{2-9}
\multicolumn{1}{c}{}                                     & \multicolumn{8}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Dataset}}                                                                                                                                                                                   \\ \cline{2-9} 
\multicolumn{1}{c}{}                                     & \multicolumn{2}{c|}{Fash. MNIST}                                 & \multicolumn{2}{c|}{CelebA}                              & \multicolumn{2}{c|}{Cat vs Dog}                         & \multicolumn{2}{c}{Imagenet}                           \\
\multicolumn{1}{c}{\multirow{-3}{*}{}}                   & \multicolumn{1}{c|}{OTNN} & \multicolumn{1}{c|}{Uncst.}          & \multicolumn{1}{c|}{OTNN} & \multicolumn{1}{c|}{Uncst.}  & \multicolumn{1}{c|}{OTNN} & \multicolumn{1}{c|}{Uncst.} & \multicolumn{1}{c|}{OTNN} & \multicolumn{1}{c}{Uncst.} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Attribution} & \multicolumn{8}{c}{\cellcolor[HTML]{EFEFEF}\textbf{$\mu\text{Fidelity-Uniform}$ ($\uparrow$ is better)}}                                                                                                                                       \\ \hline
\multicolumn{1}{l|}{Saliency}                            & \textbf{0.156}            & \multicolumn{1}{l|}{-0.001}          & \textbf{0.244}            & \multicolumn{1}{l|}{0.052}   &                   \textbf{0.091}        & \multicolumn{1}{l|}{0.080}       &           \textbf{0.240 }          &  0.004                            \\
\multicolumn{1}{l|}{GradCam}                                  & \textbf{0.215}            & \multicolumn{1}{l|}{0.02}            & \textbf{0.028}            & \multicolumn{1}{l|}{0.002}   &                    \textbf{0.101}       & \multicolumn{1}{l|}{0.052}       &          0.029                 &               \textbf{0.046 }            \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Attribution} & \multicolumn{8}{c}{\cellcolor[HTML]{EFEFEF}\textbf{$\mu\text{Fidelity-Zero}$  ($\uparrow$ is better)}}                                                                                                                                         \\ \hline
\multicolumn{1}{l|}{Saliency}                            & \textbf{0.246}            & \multicolumn{1}{l|}{0.034}           & \textbf{0.325}            & \multicolumn{1}{l|}{0.082}   & \textbf{0.121}            & \multicolumn{1}{l|}{0.079}  & \textbf{0.147}            & 0.049                      \\
\multicolumn{1}{l|}{GradCam}                                  & \textbf{0.161}            & \multicolumn{1}{l|}{0.046}           & \textbf{0.127}            & \multicolumn{1}{l|}{0.061}   & \textbf{0.136}            & \multicolumn{1}{l|}{0.049}  & 0.048                     & \textbf{0.068}             \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Attribution} & \multicolumn{8}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Stability Spearman rank ($\downarrow$ is better)}}                                                                                                                                          \\ \hline
\multicolumn{1}{l|}{Saliency}                            & \textbf{0.59}             & \multicolumn{1}{l|}{0.91}            & \textbf{0.51}             & \multicolumn{1}{l|}{0.77}    &                    \textbf{0.58}      & \multicolumn{1}{l|}{0.69}       &\textbf{0.60 }                     &        0.74                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{9}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Distance Saliency smoothgrad ($\downarrow$ is better)}}                                                                                                                                                                                                \\ \hline
\multicolumn{1}{l|}{Saliency}                            & \textbf{7.5e-03}          & \multicolumn{1}{l|}{7.0e-02}         & \textbf{3.1e-4}          & \multicolumn{1}{l|}{1.4e-1} &          \textbf{3.7e-8 }                & \multicolumn{1}{l|}{4.1e-8}       &          \textbf{3.7e-8 }                &            4.3e-8                 \\ \hline
\rowcolor[HTML]{EFEFEF} 
%\multicolumn{9}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Compression ($\downarrow$ is better)}}                                                                                                                                                                                                                 \\ \hline
%\multicolumn{1}{l|}{Saliency} &                           & \multicolumn{1}{l|}{}                                   & \textbf{9.5kb }                    & \multicolumn{1}{l|}{16.8kb}          &       \textbf{ 8.4kb}                   & \multicolumn{1}{l|}{8.9kb}       &            21.4kb             &       \textbf{20.9kb }                    \\ \hline
\end{tabular}
  \caption{Comparison of XAI metrics for different attributions methods and dataset for OTNN and unconstrained networks.}
\label{table:xaimetric}
\end{table}

==> partsv2/multiclass.tex <==

%\commentgreen{In this section, we put aside temporally the explainability to focus on the loss}.
In this section, we put aside the explainability to focus on hKR loss.
As pointed out in \cite{bethunelip}, one drawback of working with \onlyonelip~functions is that it depends strongly on the parameters of the loss. In the binary case, \losshkr ~(equation \ref{eq:reg_OT} ) has two parameters : the margin $m$ and the hinge weight $\lambda$. $\lambda$ represents the tradeoff between robustness and accuracy. When the classes are separable and the $m$ is small enough, the hinge part of the loss tends to zero. Since, the parameter $m$ is hard to choose, to we propose a new formulation of the loss as follows:


\begin{align}\label{eq:reghrk}
\begin{split}
 \mathcal{L}^{hKR}_{\lambda,\alpha}(\f) =&	\underset{\x \sim \dneg}{\mathbb{E}} \left[\f(\x)\right]-\underset{\x \sim \dpos}{\mathbb{E}}\left[\f(\x)\right]\\
 & +\lambda\left(\underset{(\x, \y) \sim \djoint}{\mathbb{E}} \left(m-\y \f(\x)\right)_+ -\alpha m\right)
	\end{split}
\end{align}

%\begin{equation}
%\label{reghrk}
%\mathcal{L}^{hKR}_{\lambda,\alpha}(f) =  \underset{\x \sim P_-}{\mathbb{E}} \left[f(\x)\right]-\underset{\x \sim P_+}{\mathbb{E}}\left[f(\x\right]  +\lambda\left(\underset{\x}{\mathbb{E}} \left(m-Yf(\x)\right)_+ +\alpha m\right)
%\end{equation}
with $m>0$ a learnable parameter,
%. In this formulation, $m$ is no more a parameter but a variable to optimize, 
and $0<\alpha \leq 1$ is a new parameter. It is easy to see that, according to the linear growth of $\alpha m$ and its opposite hinge term, if $\f(\x)$ is uniformly distributed on a bounded interval, the optimal margin $m$ is obtained when the ratio of $\x$ such that $\f(\x)\leq m$ is equal to $\alpha$. The latter  can be interpreted as the target proportion of data that is concerned by the hinge part of the loss. By choosing $\lambda \approx \frac{1}{\alpha}$, the weight of the KR part in the loss will be approximately the same as the hinge part at the end of the optimizing process. With this approach, the only parameter to choose is $\alpha$ which can be interpreted as the approximated error rate targeted in the learning process. 

%\commentgreen{Proposition de changer de titre: A mon avis, vu ce que j'ai du decrire avant, il faudra faire de cette partie une extension au multiclass avec une proposition loss, et expliquer comment on adapte d'explication basée gradient au multiclass; et dire que même si les theoreme ne s'appliquent pas directement au multiclass, on montrera des résultats interessant dans la partie experiments}

An extension has also been proposed in \cite{serrurier2021achieving} to the  multiclass case with $q$ classes. The idea is to learn $q$ \onlyonelip~functions $(\f_1, \ldots, \f_q)$, each component $\f_i$ being a  \textit{one-versus-all} binary classifier. The loss proposed was the following 


\iffalse
\begin{align}\label{eq:hkr_multi}
\begin{split}
 \mathcal{L}^{hKR}_\lambda(\f_1,\ldots,\f_q) =&
 \sum_{k=1}^q \left[\underset{\x \sim \neg P_k}{\mathbb{E}} \left[\f_k(\x)\right] -\underset{\x \sim P_k}{\mathbb{E}}\left[\f_k(\x)\right] \right]
\\ 
&+\lambda\underset{(\x,\y) \sim \underset{k=1}{\bigcup^q}P_k
 }{\mathbb{E}}(H\left(\f_1(\x),\ldots, \f_q(\x) ,\y\right)
	\end{split}
\end{align}
\fi

\begin{align}\label{eq:hkr_multi}
\begin{split}
 \mathcal{L}^{hKR}_\lambda(\f_1,\ldots,\f_q) =&
 \sum_{k=1}^q \left[\underset{\x \sim \neg P_k}{\mathbb{E}} \left[\f_k(\x)\right] -\underset{\x \sim P_k}{\mathbb{E}}\left[\f_k(\x)\right] \right]
\\ 
&+\lambda \underset{(\x,\y) \sim \djoint}{\mathbb{E}}(H\left(\f_1(\x),\ldots, \f_q(\x) ,\y\right)
	\end{split}
\end{align}


%\begin{equation}
%\label{eq:hkr_multi}
%\mathcal{L}^{hKR}_\lambda(f_1,\ldots,f_q) = \sum_{k=1}^q \left[\underset{\textbf{x}  \sim \neg P_k}{\mathbb{E}} \left[f_k(\textbf{x})\right] -\underset{\textbf{x} \sim P_k}{\mathbb{E}}\left[f_k(\textbf{x})\right] \right]
% +\lambda\underset{\textbf{x},\y\sim \underset{k=1}{\bigcup^q}P_k
% }{\mathbb{E}}(H\left(f_1(\x),\ldots, f_q(\x) ,\y\right)
%\end{equation}
with :

\begin{equation}
\label{eq:hinge_multi}
H\left(f_1(\x),\ldots, f_q(\x),\y \right) =\sum_{k=1}^q \left(m -(2*\mathbbm{1}_{y=k}-1)*\f_k(\x)\right)_+
\end{equation}



\fel{define $P_k$ here. Suggestion, we have already defined the joint $\djoint$ so we could easily say 'with $\djoint_k = \djoint(\x | \y = k)$ '. Also check with the union}
This formulation has three main drawbacks: (\textbf{\textit{i}}) the optimal margin for each class may be different leading to a huge number of hyperparameters - solved by \cref{eq:reghrk}-, (\textbf{\textit{ii}}) for a large number of classes several outputs may have few or no positive sample within a batch leading to slow convergence, (\textbf{\textit{iii}})  weight of $\f_y(\x)$ (the function of the true class) with respect to the other decreases when the number of classes increases. To overcome these drawbacks, we propose a softmax-based hinge regularization with a learnable margin :

\begin{align}\label{eq:Hingesoft}
\begin{split}
 H^{\alpha}_{soft}&\left(\f_1(\x),\ldots, \f_q(\x),\y \right) 	=\\
 &\left(m_y-\frac{1}{2} \f_y(\x)+\frac{1}{2} \sum_{k\neq y} \f_k(\x)*\frac{e^{\f_k(\x)}}{\sum_{j\neq y} e^{\f_j(\x)}}\right)_+\\
 & - \alpha  m_y
	\end{split}
\end{align}


%\begin{equation}
%\label{eq:Hingesoft}
%H^{\alpha}_{soft}\left(f_1(\x),\ldots, f_q(\x),\y \right) =m_y-\frac{1}{2} f_y(\x) +\frac{1}{2} \sum_{k\neq y} f_k(\x)*\frac{e^{f_k(\x)}}{\sum_{j\neq y} e^{f_j(\x)}} + \alpha  m_y
%\end{equation}
with $m_y\geq 0$ and 
%\begin{equation}
%soft(f_k(\x)) = \frac{e^{f_k(\x)}}{\sum_{j\neq y} e^{f_j(\x)}}
%\end{equation}
 in this function, the value of $\f_{\y}(\x)$ for the true class  always has the same weight as the value of the other functions, no matter the number of classes. At the beginning of the learning, the softmax acts like an average since all the values of $\f_k$ are close. During the learning process, the values of $\f_k$ diverge and the softmax acts like a maximum.  Margins are automatically learnt as for the binary case ($\alpha$ a single hyperparameter).

==> partsv2/qualitative_results_otml.tex <==
Using the learnt \otnn~on  CelebA (Mouth Slightly Open label), Cat vs Dog and Imagenet, Fig.~\ref{fig:celebA_counterfactual}  presents the original image, average gradients $\nabla_x f_j$  over the channels, and images in the direction of the transport plan (Prop.~\ref{th:gradient_transport_plan}), other samples and datasets are given in Appendix~A.5. 
We can see that most of the gradients are visually consistent, showing clearly what has to be changed in the input image to modify the class and act as a counterfactual explanation. 
%what needed to change in the input image to classes and act as a counterfactual explanation. 
This is less clear for the Imagenet examples. This could be due to the difficulty of defining a transport plan for each pair of the 1000 classes. However, feature visualizations in Figure \ref{fig:big_picture} show that the internal representation of the classes is still more interpretable than the unconstraint one. 
More generally, we observe that the gradient gives clear information about how the classifier makes its decision. For instance, for the cat, it shows that the classifier does not need to encode perfectly the concept of a cat, but mainly to identify the color of the eyes and size of the nose.
%\commentgreen{@Mathieu tu en feras d'autres images sinon enlever la paranthese}

\iffalse
\begin{figure*}
\centering
\begin{tabular}{ccc}
\multicolumn{3}{c}{CelebA Mouth Slightly Open label: left close to open, right open to close} \\
  \begin{tabular}{lll}
\includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00024_input_lbl0_fx-0.59.png} & \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00024_gradColor.png} & \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00024_xMinus10.0Grad.png} 
 \end{tabular} &
  \begin{tabular}{lll}
\includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00072_input_lbl1_fx0.47.png} & \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00072_gradColor.png} & \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00072_xMinus10.0Grad.png} 
 \end{tabular} & \\
 %\midrule
\multicolumn{3}{c}{Cat vs Dog : left cat to dog, right dog to cat} \\
  
\includegraphics[width=.5\linewidth] {img/catvsdog/expl_1.jpg} &
  \includegraphics[width=.5\linewidth] {img/catvsdog/expl_2.jpg} & \\
% \midrule
\multicolumn{3}{c}{Imagenet :left cabbage butterfly to monarch one,  right great grey owl to bald eagle} \\
  \includegraphics[width=.5\linewidth] {img/imagenet/expl_1.jpg} &
  \includegraphics[width=.5\linewidth] {img/imagenet/expl_2.jpg} %\\
& \\
 \end{tabular}
\caption{Samples of conterfactuals from different dataset: (left) source image , (center) gradient image, (right) counterfactual of the form $\x-t*\hat{f}(\x)\nabla_x \hat{f}(\x)$, for  $t>1$}
\label{fig:celebA_counterfactual}
\end{figure*}


\begin{figure*}[h]
  \centering
  \fbox{\includegraphics[width=0.98\linewidth]{img/fashion-otnn.png}}
  
\caption{Samples from different classes of FashionMNIST: (left) source image , (center) targeted gradient image of an \otnn, (right) targeted counterfactual of the form $\x-10*\hat{f}(\x)\nabla_x \hat{f}(\x)$}
%Counterfactuals of the form $ \x-10*\hat{f}(\x)\nabla_x \hat{f}(\x)$  of a \otnn~ for FashionMNIST. }
\label{fig:fashion_mnist}
\end{figure*}
\fi

\iftrue
\begin{figure*}
    \centering
    \begin{tabular}{rcc}
        %\multicolumn{3}{c}{Fashion MNIST source image and class, targeted gradient image and counterfactual.} \\
        %\multicolumn{3}{c}{\includegraphics[width=1.0\linewidth]{img/fashion-otnn.pdf}}\\
        %\multicolumn{3}{c}{CelebA Mouth Slightly Open label: left close to open, right open to close} \\
        \rotatebox[origin=c]{90}{CelebA}\hspace{-5mm} & 
        \begin{tabular}{ccc}
            \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00024_input_lbl0_fx-0.59.pdf} & \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00024_gradColor.pdf} & \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00024_xMinus10.0Grad.pdf}\\
            % \textbf{mouth closed} & $\to$ & \textbf{mouth opened}
        \end{tabular} &
        \begin{tabular}{ccc}
            \hspace{-4mm}
            \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00072_input_lbl1_fx0.47.pdf} & \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00072_gradColor.pdf} & \includegraphics[width=.13\linewidth]{img/Mouth_slightly_open/00072_xMinus10.0Grad.pdf} \\
            % \textbf{mouth opened} & $\to$ & \textbf{mouth closed}
        \end{tabular} \\
          & \textbf{mouth closed $\to$ mouth opened} &  \textbf{mouth opened $\to$ mouth closed}\\
        %\midrule
        % \multicolumn{3}{c}{CelebA Blurry label: left blurry to not blurry, right not blurry to blurry} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=c]{90}{CelebA}\hspace{-5mm} & 
        \begin{tabular}{ccc}
            \includegraphics[width=.13\linewidth]{img/samplesAppendix/Blurry/00027_input_lbl1_fx0.72.pdf} & \includegraphics[width=.13\linewidth]{img/samplesAppendix/Blurry/00027_gradColor.pdf} & \includegraphics[width=.13\linewidth]{img/samplesAppendix/Blurry/00027_xMinus10.0Grad.pdf}\\
            % \textbf{blurry} & $\to$ & \textbf{not blurry}
        \end{tabular} &
        \begin{tabular}{ccc}
            \hspace{-4mm}
            \includegraphics[width=.13\linewidth]{img/samplesAppendix/Blurry/00250_input_lbl0_fx-1.15.pdf} & \includegraphics[width=.13\linewidth]{img/samplesAppendix/Blurry/00250_gradColor.pdf} & \includegraphics[width=.13\linewidth]{img/samplesAppendix/Blurry/00250_xMinus5.0Grad.pdf}\\
            % \textbf{not blurry} & $\to$ & \textbf{blurry}
        \end{tabular} \\
          & \textbf{blurry $\to$ not blurry} & \textbf{not blurry $\to$ blurry}\\
        %\midrule
        % \multicolumn{3}{c}{CelebA Rosy cheeks label: rosy to not rosy, right not rosy to rosy} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=c]{90}{CelebA}\hspace{-5mm} & 
        \begin{tabular}{ccc}
            \includegraphics[width=.13\linewidth]{img/samplesAppendix/Rosy_Cheeks/00132_input_lbl1_fx3.26.pdf} & \includegraphics[width=.13\linewidth]{img/samplesAppendix/Rosy_Cheeks/00132_gradColor.pdf} & \includegraphics[width=.13\linewidth]{img/samplesAppendix/Rosy_Cheeks/00132_xMinus2.5Grad.pdf}\\
            % \textbf{rosy cheeks} & $\to$ & \textbf{w/o rosy cheeks}
        \end{tabular} &
        \begin{tabular}{ccc}
            \hspace{-4mm}
            \includegraphics[width=.13\linewidth]{img/samplesAppendix/Rosy_Cheeks/00079_input_lbl0_fx-7.52.pdf} & \includegraphics[width=.13\linewidth]{img/samplesAppendix/Rosy_Cheeks/00079_gradColor.pdf} & \includegraphics[width=.13\linewidth]{img/samplesAppendix/Rosy_Cheeks/00079_xMinus2.0Grad.pdf}\\
            % \textbf{w/o rosy cheeks} & $\to$ & \textbf{rosy cheeks}
        \end{tabular} \\
        & \textbf{rosy cheeks $\to$ w/o rosy cheeks} & \textbf{w/o rosy cheeks $\to$ rosy cheeks}\\
        %\midrule 
        %\multicolumn{3}{c}{Cat vs dog : left cat to dog, right dog to cat} \\
        \rotatebox{90}{\quad Cat vs Dog}\hspace{-5mm} &
        \includegraphics[width=.464\linewidth] {img/catvsdog/expl_1.jpg} &
            \hspace{-4mm}
        \includegraphics[width=.464\linewidth] {img/catvsdog/expl_2.jpg}\\
        & \textbf{cat $\to$ dog} & \textbf{dog $\to$ cat}\\
        % \midrule
        % \multicolumn{3}{c}{Imagenet :left cabbage butterfly to monarch one,  right great grey owl to bald eagle} \\
        \rotatebox{90}{\quad Imagenet}\hspace{-5mm} &
        \includegraphics[width=.464\linewidth] {img/imagenet/expl_1.jpg} &
            \hspace{-4mm}
        \includegraphics[width=.464\linewidth] {img/imagenet/expl_2.jpg} \\
        & \textbf{cabbage butterfly $\to$ monarch butterfly} & \textbf{great grey owl $\to$ bald eagle}\\
     \end{tabular}
    \caption{Samples of counterfactuals from different datasets: (left) source image , (center) gradient image, (right) counterfactual of the form $\x-t*\hat{f}(\x)\nabla_x \hat{f}(\x)$, for  $t>1$}
    \label{fig:celebA_counterfactual}
\end{figure*}
\fi



==> partsv2/related_work_otml.tex <==
\textbf{1-Lipschitz Neural network and optimal transport:}
%
%For sake of simplicity, we consider binary classification problems on feature vector space $\X \subseteq \Omega$ and labels $\Y = \{-1,1\}$. We name $P_+=\mathbb{P}(X|Y=1)$ and  $P_-=\mathbb{P}(X|Y=-1)$, the conditional distributions with respect to Y. We note $p=P(Y=1)$ and $1-p=P(Y=-1)$ the apriori class distribution. \\
%\fel{@louis: check ce que j'ai fait ici quand tu peux.}
Consider a classical supervised machine learning binary classification problem on $(\Omega, \mathcal{F}, \mathbb{P})$ -- the underlying probability space -- where $\Omega$ is the sample space, $\mathcal{F}$ is a $\sigma$-algebra on $\Omega$, and $\mathbb{P}$ is a probability measure on $\mathcal{F}$. 
%
We denote the input space $\inp \subseteq \mathbb{R}^d$ and the output space $\mathcal{Y} = \{\pm 1 \}$. Let input data $\x : \Omega \to \inp$ and target label $\y : \Omega \to \mathcal{Y}$ are random variables with distributions $\dx$, $\dy$, respectively.
%
The joint random vector $(\x, \y)$ on $(\Omega, \mathcal{F})$ has a joint distribution $\djoint$ defined over the product space $\inp \times \mathcal{Y}$.
%
Moreover, let $\dpos = \djoint(\x | \y = 1)$ and $\dneg = \djoint(\x | \y = -1)$ the conditional probability distributions of $\x$ given
%that the true label is positive or negative, respectively. 
the true label.
We assume that the supports of $\Omega$,  $\dpos$ and $\dneg$ are compact sets.


%The classification problem is balanced when $p=\frac{1}{2}$.\\
A function $\f :\inp \to \mathbb{R}$ is a 1-Lipschitz functions over $\inp$ (denoted $Lip_1(\inp)$) if and only if $\forall (\x,\z) \in \inp^2, ||\f(\x) -\f(\z) ||\leq || \x-\z||$.
\onlyonelip~neural networks have received a lot of attention, especially due to the link with adversarial attacks. They provide certifiable robustness guarantees~\cite{hein_formal_2017,ono_lightweight_2018}, improve  the generalizations~\cite{Sokolic_2017} and the interpretability of the model~\cite{tsipras2018robustness}. The simplest way to constrain a network to be in $Lip_1(\inp)$ is to impose this \onlyonelip~property to each layer. Frobenius normalization \cite{SalimansK16}, or spectral normalization \cite{Miyato2018SpectralNF} can be used for linear layers, and can also be extended, in some situations, to  orthogonalization \cite{li2019preventing,Achour2021}.
%\commentgreen{peut etre ajouter le papier de elmehdi pour l'instant que sur arxiv mais d'ici la jmlr}

Optimal transport, \onlyonelip~neural networks, and binary classification were first associated in the context of Wasserstein GAN (WGAN) \cite{Arjovsky2017}. The discriminator of a WGAN is the solution to the Kantorovich-Rubinstein dual formulation of the $1$-Wasserstein distance \cite{villani2008}, and it can be regarded as a binary classifier with a carefully chosen threshold.
Nevertheless, it has been demonstrated in \cite{serrurier2021achieving} that this type of classifier is suboptimal, even on a toy dataset. In the same paper, the authors address the suboptimality of the Wasserstein classifier by introducing the hKR loss $\mathcal{L}^{hKR}$, which adds a hinge regularization term to the Kantorovich-Rubinstein optimization objective~:
\begin{equation} \label{eq:reg_OT} 
\mathcal{L}^{hKR}_{\lambda,m}(\f) =  \underset{\x \sim \dneg}{\mathbb{E}} \left[\f(\x)\right]-\underset{\x \sim \dpos}{\mathbb{E}}\left[\f(\x)\right]  +\lambda\underset{(\x, \y) \sim \djoint}{\mathbb{E}} \left(m-\y \f(\x)\right)_+ 
\end{equation}
where $m>0$ is the margin, and  $(z)_+ = max(0,z)$. We note $\f^*$ 
the optimal minimizer of $\mathcal{L}^{hKR}_{\lambda,m}$. The classification is given by the sign of $\f^*$. In the following, the \onlyonelip~neural networks that minimize $\mathcal{L}^{hKR}_{\lambda,m}$ will be denoted as \otnn.
%MAthieu : on l'a déjà fait dans l'intro mais bon
~Given a function $\f$, a classifier based on $\sign(\f)$ and an example $\x$, an adversarial example is defined as follows:
\begin{align}
    &adv(\f, \x) = \argmin_{\z \in \inp} \parallel \x -\z \parallel 
    ~~ s.t. ~~ \sign(\f(\z)) \neq \sign(\f(\x)) .
    \label{def:adversary}
\end{align}
Since $\f^*$ is a \onlyonelip~function, $|\f^*(\x)|$ is a certifiable lower bound of the robustness of the classification of $\x$ 
(i.e. $\forall \x \in \inp, |\f^*(\x)|\leq ||\x - adv(\f^*,\x) || $). The function $\f^*$ has the following properties \cite{serrurier2021achieving}
~(\textbf{\textit{i}}) if the supports of $\dpos$ and $\dneg$ are disjoints (separable classes) with a minimal distance of $\epsilon>0$, then for $m<2\epsilon$, $f^*$ 
achieves 100\% accuracy; % on $\dpos$ and $\dneg$ \fel{mu et nu (avnt P+ et P-) sont des proba distrib. je changerai separable (meme si je comprend ce que tu veux dire) };
~(\textbf{\textit{ii}}) minimizing $\mathcal{L}^{hKR}$ is still the dual formulation of an optimal transport problem (see appendix for more details).

\textbf{Explainability and metrics:} 
Attribution methods aim to explain the prediction of a deep neural network by pointing out input variables that support the prediction -- typically pixels or image regions for images -- which lead to importance maps.
%Attribution methods aims to provide a rank of important variables in the decision of a classfier. 
Saliency~\cite{SimonyanVZ13} was the first proposed white-box attribution method and consists of back-propagating the gradient from the output to the input. The resulting absolute gradient heatmap indicates which pixels affect the most the decision score.
However, this family of methods suffers from problems inherent to the gradients of standard models. These methods were then followed by a plethora of other methods as Integrated Gradient~\cite{Sundararajan2017}, SmoothGrad~\cite{Smilkov2017}, Grad-cam~\cite{Selvaraju_2019}, Input Gradient~\cite{ancona18GradInput}.

%others methods aim to explore perturbations around the image to measure the variation of the classification output and build an importance map~\cite{petsiuk18Rise,fel21sobol}. 
%followed by several improvements such as Grad-cam~\cite{Selvaraju_2019},Gradient.Input~\cite{ancona18GradInput}, Integrated Gradients~\cite{Sundararajan2017}, Smoothgrad~\cite{Smilkov2017}, all relying on gradient calculation of the classifcation method. 

%\fel{Proposition (metrics): 
However, it is becoming increasingly clear that current methods raise many issues~\cite{Adebayo18Sanity, Heo19foolingInterpretation, sixt2020explanations} such as confirmation bias: it is not because the explanations make sense to humans that they reflect the evidence of the prediction. 
To address this challenge, a large number of metrics were proposed to provide objective evaluations of the quality of explanations. Deletion and Insertion methods~\cite{petsiuk18Rise} evaluate the drop in accuracy when important pixels are replaced by a baseline. $\mu\text{Fidelity}$ method~\cite{Bhatt20muFidelity} evaluates the correlation between the sum of importance scores of pixels and the drop of the score when removing these pixels.
%Finally, 
Other metrics 
%propose to assess other
consider properties such as generalizability, consistency~\cite{felHowGood22}, or stability~\cite{Yeh19InfidelityExplain,Bhatt20muFidelity} of explanation methods.
A recent approach~\cite{linsley2017visual} aims to evaluate the alignment between attribution methods and human feature importance across 200,000 unique ImageNet images (called ClickMe dataset). The alignment between DNN Saliency and human explanations is quantified using the mean Spearman correlation, normalized by the average inter-rater alignment of humans.
%\mathieu{The ClickMe dataset~\cite{linsley2017visual} allows for the evaluation of the alignment between attribution methods and human feature importance across 200,000 unique ImageNet images. In their study \cite{fel2022aligning}, the authors utilize this dataset to illustrate the trade-off between deep neural network (DNN) performance and alignment with human feature importance.. The alignment between human and DNN saliency is quantified using the mean Spearman correlation, normalized by the average inter-rater alignment of humans.}


These works on explainability metrics have also initiated the emergence of links between the robustness of models and the quality of their explanations~\cite{Chalasani20explanationAdvTraining,wang2022robust}. In particular,\cite{felHowGood22} claimed that \onlyonelip~networks explanations have better metrics scores. But this study was not on \otnn s~and was limited to their proposed metrics.

To end with, recent literature is focusing on  counterfactual explanations \cite{wachter2017counterfactual,Verma20CounterfactualReview} methods, providing information on "why the decision was A and not B". Several properties are desirable for these counterfactual explanations\cite{Verma20CounterfactualReview}: Validity (close sample and in another class), Actionability, Sparsity, Data Manifold closeness, and Causality.
The three last properties are generally not covered by standard adversarial attacks and complex methods have been proposed~\cite{Goyal19counter,rodriguez21beyond,wang20scout}. %For the causality property, recent papers~\cite{black19OptimTransp,deLara2021} have proposed, when a causal model is hard to fully-defined , a definition of optimal transport based counterfactuals easier to compute and that can sometimes coincide with causal model based ones. 
Since often a causal model is hard to fully-define, recent papers~\cite{black19OptimTransp,deLara2021} have proposed a definition of counterfactual based on optimal transport easier to compute and that can sometimes coincide with causal model based ones. 
We will rely on this theoretical definition of counterfactuals.

==> partsv2/table_fidelity.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.87}{
        \begin{tabular}{l C{0mm} P{0mm} P{5mm}P{5mm}P{5mm}P{5mm}P{5mm} P{1mm} P{5mm}P{5mm}P{9mm}P{5mm}P{5mm} P{1mm} P{5mm}P{5mm}P{5mm}P{5mm}P{5mm}}
        \toprule
        &&& \multicolumn{5}{c}{MNIST} &&  \multicolumn{5}{c}{Cifar-10} &&  \multicolumn{5}{c}{ImageNet}  \\
        \cmidrule(lr){4-8} \cmidrule(lr){10-14} \cmidrule(lr){16-20}
        
        &&& Del.$\downarrow$ & Ins.$\uparrow$ & Fid.$\uparrow$ & Rob.$\downarrow$ & Time 
        && Del.$\downarrow$ & Ins.$\uparrow$ & Fid.$\uparrow$ & Rob.$\downarrow$ & Time 
        && Del.$\downarrow$ & Ins.$\uparrow$ & Fid.$\uparrow$ & Rob.$\downarrow$ & Time
        \\
        
        \midrule
        Saliency\cite{simonyan2013deep} &   && .193 & \underline{.633} & \underline{.378} & .071 & 0.04
                 && \underline{.171} & .172 & -.021 & .026 & 0.16
                 && \underline{.057} & .126 & .035 & .769 & 0.36 \\
        GradInput\cite{ancona2017better} &   && .222 & .611 & .107 & .074 & 0.04 
                 && .200 & .143 & -.018 & .095 & 0.17
                 && \underline{.057} & .050 & .023 & .814 & 0.36  \\
        SmoothGrad\cite{smilkov2017smoothgrad} &   && .185 & .621 & .331  & .070 & 1.91
                 && .174 & .181 & .092 & .048 & 9.07
                 && \textbf{.051} & .069 & .019 & .809 & 9.63 \\
        VarGrad\cite{seo2018noise} &   && .207   & .555   & .216   & .077   & 1.76 
                 && .183 & .211 & -.012 & .193 & 9.07
                 && .098 & .201 & .021 & .787 &  9.62 \\
        InteGrad\cite{sundararajan2017axiomatic} &   && .209 & .615 & .108 & .074 & 1.77
                 && .194 & .171 & -.016 & .154 & 7.19
                 && .058 & .052 & .023 & .813 & 8.39 \\
        Occlusion\cite{ancona2017better} &   && .247  & .545  & .137  & .082  & 0.04 
                 && .217 & \underline{.290} & .105 & .232 & 1.13
                 && .100 & .266 & .026 & .821 & 4.97 \\
        GradCAM\cite{Selvaraju_2019} &   && n/a &  n/a  &  n/a  &  n/a  &  n/a  
                 && .297 & .282 & .056 & .195 & 0.39
                 && .073 & .232 & .036 & .817 & 0.18 \\
        GradCAM++\cite{chattopadhay2018grad} &   && n/a  & n/a & n/a & n/a & n/a
                 && .270 & \textbf{.326} & .102 & .094 & 0.39
                 && .074 & \underline{.285} & \underline{.054} & .800 & 0.19 \\
        RISE\cite{petsiuk2018rise}     &   && .248  & .558 & .133  & .093  & 2.26 
                 && .196 & .273  & \underline{.157} & .385 & 20.5
                 && .074 & .276 & \textbf{.154} & .818 & 1215 \\
        Greedy-AS\cite{hsieh2020evaluations} &   && .260  & .497  & .110  & \textbf{.061}  & 335
                 && .205 & .264 & -.003 & \textbf{.013} & 4618
                 && .088 & .047 & .023 & \textbf{.612} & 180056  \\
        \midrule 
        %Greedy-AO && .237 & .572 & .244 & \underline{.063} & 290
        %         && \textbf{.162} & .283 & .041 & .024 & 2874
        %         && .086 & .050 & .023 & \underline{.752} & 26762 \\
        %\evaEmp  && \underline{.101} & .621 & \underline{.378} & .067 & 14.4 
        %         && .184 & .270 & \textbf{.397} & \underline{.022} & 186.6
        %         && \multirow{ 2}{*}{.070} & \multirow{ 2}{*}{\textbf{.289}} & \multirow{ 2}{*}{.048} & \multirow{ 2}{*}{.758} & \multirow{ 2}{*}{6454} \\ 
        %\eva     && \textbf{.089} & \textbf{.736} & \textbf{.428} & .069 & 1.29 
        %         && \underline{.164} & \underline{.290} & \underline{.352} & .025 & 12.7 \\
                 %&& .070 & \textbf{.289} & \underline{.048} & \underline{.758} &  \\
        \textbf{\eva}~(ours)     & && \textbf{.089} & \textbf{.736} & \textbf{.428} & \underline{.069} & 1.29 
                 && \textbf{.164} & \underline{.290} & \textbf{.352} & \underline{.025} & 12.7 
                 && .070 & \textbf{.289} & .048 & \underline{.758} & 6454
                 \\
        
        \bottomrule \\
        \end{tabular}
    }
    \caption{Results on Deletion (Del.), Insertion (Ins.), $\mu$Fidelity (Fid.) and \rsr~ (Rob.) metrics. 
Time in seconds corresponds to the generation of 500 (MNIST/CIFAR-10) and 100 (ImageNet) explanations on an Nvidia P100.
Note that \eva~is the only method with guarantees that the entire set of possible perturbations has been exhaustively searched.
Verified perturbation analysis with IBP + Forward + Backward is used for MNIST, with Forward only for  CIFAR-10 and with our hybrid strategy described in Section.\ref{sec:scaling} for ImageNet. 
Grad-CAM and Grad-CAM++ are not calculated on the MNIST dataset since the network  only has dense layers. 
%Greedy-AO is the equivalent of Greedy-AS but with the \AO estimator. 
%\fel{rajouter colonne certifiable ? Avec des croix rouges sauf nous, remove greedy-ao, mettre (ours) a cote de eva}
%For ImageNet, we used the hybrid approach described in \ref{sec:scaling}.
The first and second best results are  in \textbf{bold} and \underline{underlined}, respectively. 
}
    \label{tab:cifar_mnist_metrics}
    \vspace{-3mm}
\end{table*}

==> partsv2/transport_robustness_otml.tex <==
In this section, we extend the properties of the \otnn s~to the explainability framework, all the proofs are in the appendix~A.1. We note $\pi$ the optimal transport plan corresponding to the minimizer of \losshkr. In the most general setting, $\pi$ is a joint distribution over $\dpos,\dneg$ pairs. However when $\dpos$ and $\dneg$ admit a density function~\cite{peyre2018computational} with respect to Lebesgue measure, then the joint density describes a deterministic mapping, i.e. a Monge map. Given $\x \sim \dpos$ %\fel{check here, belong to with proba distrib. (sugg: $\x \sim \dpos$)} 
(resp. $\dneg$) we note $\z = \tr_\pi(\x) \in \dneg$ (resp. $\dpos$) the image of $\x$ with respect to $\pi$. When $\pi$ is not deterministic (on real datasets that are defined as a discrete collection of Diracs), we take $\tr_\pi(\x)$ as the point of maximal mass with respect to $\pi$.%\mathieu{Eventuellement utiliser que le transport est point par point si les distrib admettent une pdf}

% \fel{$\x \sim \dpos$ est correct, mais pas $\x \in \dpos$ (P+ avant) il faut qu'on reformule (meme si je comprend ce que tu veux dire). Je propose un truc du style $\sign(\f(\x)) \neq \sign(\f(\tr(\x))$?}. \commentgreen{y etait le label ds la section precedente, peut etre z. et tr n'est pas definit avant}% retirer ?

\begin{proposition}[Transportation plan direction]\label{th:gradient_transport_plan}
Let $\f^*$ an optimal solution minimizing the \losshkr. Given $\x \sim \dpos$ (resp. $\dneg$)  and  $\z = \tr_\pi(\x)$, then $\exists t \geq 0$ (resp. $t \leq 0$) such that $\tr_\pi(\x) = \x  -t \nabla_{\x}  \f^*(\x)$ almost surely. 
\end{proposition}

This proposition also holds for the Kantorovich-Rubinstein dual problem without hinge regularization, demonstrating that for $\x \sim \djoint$,
%\fel{union of proba distrib is not correct. I have properly defined $\dx$ at the beginning, I suggest $\x \sim \dx$ and $(\x,\y) \sim \djoint$ for the joint ? }
 the gradient $\nabla_{\x} \f^{*}(\x)$ indicates the direction in the transportation plan almost surely.

\begin{proposition}[Decision boundary]\label{boundary_distance}
Let $\dpos$ and $\dneg$ two distributions with disjoint supports with minimal distance~$\epsilon$ and  $\f^*$ an optimal solution minimizing the \losshkr~with $m<2\epsilon$. Given $\x \sim \djoint$, %\fel{belong to with proba distrib is not correct, c'est plutot $\x \sim \dx$? (et union non plus) mais j'ai définis $\dx$ que tu peut utiliser}, 
$\x_\delta = \x -\f^*(\x) \nabla_{\x} \f^*(\x) \in \boundary $
where $\boundary = \left\{\x' \in \inp | \f^*(\x') = 0 \right\}$  is the decision boundary (i.e. the 0 level set of $\f^*$).
\end{proposition}

 Experiments suggest this probably remains true when the supports of $\dpos$ and $\dneg$  are not disjoint. % \fel{again check here with separability}.
%, but we haven't proven it yet.\commentgreen{Je le mettrai plus positif dans l'autre sens: We will show in the experiments that this property remains true even when $P_+$ and $P_-$  are not separable.}
%\commentgreen{As said before, tu l'as déjà dit}, For any \onlyonelip~binary classifier $f$, \commentgreen{ a direct consequence of the Lipschitz property is that $|f(\x)|$ provides an upper bounf of the robustness certificate.} \sout{it is well known that the robustness certificate is higher than $|f(\x)|$ due to the Lipschitz property.}
Prop.~\ref{boundary_distance} proves that for an \otnn~ $\f$ learnt by minimizing  the \losshkr, $|\f(\x)|$ provides a tight robustness certificate. A direct consequence of~\ref{boundary_distance}, is  that $t$ defined in~\ref{th:gradient_transport_plan} is such that $|t|\geq|\f^*(\x)|$.

\begin{corollary}\label{fx_grad_adversarial}
Let $\dpos$ and $\dneg$ two separable distributions with minimal distance $\epsilon$ and  $\f^*$ an optimal solution minimizing the \losshkr~with $m<2\epsilon$, given $\x \sim \djoint$,  %\fel{$\x \sim \dx$}, 
$adv(\f^*,\x) = \x_{\delta}$ % = x-|f^*(x)|\nabla_x f^*(\x)$$ 
almost surely, where $\x_\delta = \x -\f^*(\x) \nabla_{\x} \f^*(\x)$ .
\end{corollary}

This corollary shows that adversarial examples are precisely identified for the classifier based on \losshkr: the direction given by $\nabla_{\x} \f^*(\x)$ and distance by $|\f^*(\x)|*||\nabla_{\x} \f^*(\x)||=|\f^*(\x)|$. In this scenario, the optimal adversarial attacks align with the gradient direction (i.e., FGSM attack \cite{Goodfellow2014a}). This supports the observations made in \cite{serrurier2021achieving}, where all attacks, such as PGD \cite{Madry2017} or Carlini and Wagner \cite{carlini2017towards}, applied on an \otnn~model, were equivalent to FGSM attacks.

To illustrate these propositions, we learnt a dense binary classifier with \losshkr~to separate two complex distributions, following two concentric Koch snowflakes. Fig.\ref{fig:koch}-a shows the two distributions (blue and orange snowflakes), the learnt boundary ($0$-levelset) (red dashed line). Fig.\ref{fig:koch}-{b,c} show for random samples $\x$ from the two distributions, the segments $[\x,\x_\delta]$ where $\x_\delta$ is defined in Prop.~\ref{boundary_distance} . %\sout{As expected by theorems \ref{th:gradient_transport_plan} and \ref{boundary_distance} since the attacks in the direction of the gradient follow the transport plan path and falls exactly on the decision boundary.}
As expected by Prop.~\ref{boundary_distance},  $\x_\delta$ points fall exactly on the decision boundary. Besides, as stated in Prop.~\ref{th:gradient_transport_plan} each segment provides the direction of the image with respect to the transport plan.

Finally, we showed that with \otnn, adversarial attacks are formally known and simple to compute.
%, but also corresponding to travel along a transportation map from a class to its other one. Intuitively,it means that it is not \commentgreen{
%Furthermore, since we proved that these attacks are along the transportation map, they are no more an imperceptible modification but an understandable transformation of the example.
Furthermore, since we proved that these attacks are along the transportation map, they acquire a meaningful interpretation and are no longer mere adversarial examples exploiting local noise, but rather correspond to the global solution of a transportation problem.
\section{Link between OTNN gradient and counterfactual explanations}

The vulnerability of traditional networks to adversarial attacks indicates that their decision boundaries are locally flawed, deviating significantly from the Bayesian boundaries between classes. Since the gradient directs towards this anomalous boundary, Saliency Maps~\cite{SimonyanVZ13}, given by $ \bm{g}(\x) = | \nabla_{\x} \f(\x) | $ fails to represent a meaningful transition between classes and then often lead to noisy explanation (as stated in Section~\ref{sec:related_work}).

On the contrary, in the experiments, we will demonstrate that OTNN gradients induce meaningful explanations (Sec.~\ref{sec:experiments}). We justify these good properties by building a  link with counterfactual explanations. Indeed, according to~\cite{black19OptimTransp,deLara2021}, optimal transport plans are potential surrogates or even substitutes to causal counterfactuals.  Optimal Transport plan provides for any sample $\x \in \dpos$ a sample $\tr_\pi(\x)\in  \dneg$, the closest in average on the pairing process. ~\cite{deLara2021} prove that these optimal transport plans can even coincide with causal counterfactuals when available.
Relying on this definition of OT counterfactual, Prop.~\ref{th:gradient_transport_plan} demonstrates that 
gradients 
%$\nabla_{\x}  \f^*(\x)$
 of the optimal OTNN solution 
%\otnn s~gradients  $\nabla_{\x}  \f^*(\x)$ 
provide almost surely the direction to the counterfactual $\tr_\pi(\x) = \x-t\nabla_{\x} \f^*(\x)$. Even if $t$ is only partially known, using $t = \f^*(\x)$, we know that $\x_\delta$ is on the decision boundary (Corr.~\ref{fx_grad_adversarial}) and is both an adversarial attack and a counterfactual explanation and $|t|\geq |\f^*(\x)|$ is on the path to the other distribution.
%optimal transport plan.
\\
Thus the learning process of  \otnn s~induces a strong constraint on the gradients of the neural network, aligning them to the optimal transport plan. We claim that is the reason why the simple Saliency Maps for \otnn s~have very good properties: We will demonstrate in the Sec~\ref{sec:experiments} that, for the Saliency Map explanations: (\textbf{\textit{i}}) metrics scores are higher  or comparable to other explanation methods (which is not the case for unconstrained networks), thus it has higher ranks; (\textbf{\textit{ii}}) distance to other attribution methods such as Smoothgrad is imperceptible; (\textbf{\textit{iii}})
scores obtained on metrics that can be compared between networks are higher than those obtained with unconstrained networks; (\textbf{\textit{iv}}) alignment with human explanations is impressive.

%\sout{
%In the following, we will take advantage of these properties to show that 
%$\nabla_{\x} \f^*(\x)$ provides a natural counterfactual explanation with provable explainability properties.
%}

\begin{figure*}
\centering
\includegraphics[width=.9\textwidth]{img/koch_v4.pdf}
\caption{Level sets of an \otnn~classifier $\f$ for two concentric Koch snowflakes (a).  The decision boundary (denoted $\boundary$, also called the 0-level set) is the red dashed line. Figure (b) (resp. (c)) represents 
the translation of the form $\x'= \x-\f(\x)\nabla_{\x} \f(\x)$  of each point $\x$ of the first class (resp second class). 
$[\x,\x']$ pairs are represented by blue (resp. orange)  segments.}
\label{fig:koch}
\end{figure*}




